Reliable Broadcast in Practical Networks: Algorithm and Evaluation

Reliable broadcast is an important primitive to ensure that a source node can reliably disseminate a message to all the non-faulty nodes in an asynchronous and failure-prone networked system. Byzantine Reliable Broadcast protocols were first proposed by Bracha in 1987, and have been widely used in fault-tolerant systems and protocols. Several recent protocols have improved the round and bit complexity of these algorithms. Motivated by the constraints in practical networks, we revisit the problem. In particular, we use cryptographic hash functions and erasure coding to reduce communication and computation complexity and simplify the protocol design. We also identify the fundamental trade-offs of Byzantine Reliable Broadcast protocols with respect to resilience (number of nodes), local computation, round complexity, and bit complexity. Finally, we also design and implement a general testing framework for similar communication protocols. We evaluate our protocols using our framework. The results demonstrate that our protocols have superior performance in practical networks.

==> crash.tex <==
\section{Warm-up: Crash-tolerant RB}



\begin{comment}
\subsection{Old Algorithm -- forgot where it's from.}

\begin{algorithm}[H]
\caption{Reliable Broadcast for node $j$ with message $m$ of index $h$}
\begin{algorithmic}[1]
\Function{Reliable-Broadcast}{$m, h$}
    \State {\sc Send}($\msg, j, m, h$) to all nodes  
\EndFunction
\end{algorithmic}
\end{algorithm}

\roger{$j'$ here bears some explanation: such a node $j'$ may not be the source node $j$ that initially sends $(m, j)$}. 

\lewis{Maybe we should change the source to $s$? That makes more sense to me.}

\begin{algorithm}[H]
\caption{Reliable Accept for node $i$ when receiving from node $j'$}
\begin{algorithmic}[1]
\Function{Receiving}{$\msg, j, m, h$}
    \If{never sent $(\msg,j,m,h) $}
    \State {\sc Send}($\msg, j, m, h$) to all nodes   
    \State {\sc Reliable-Accept($j,m,h$)}
    \EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{Coded Version}
\end{comment}

In this section, we present a simple idea that augments the original crash-tolerant reliable broadcast (CRB) \cite{XXX} with erasure coding. The new protocol is named \textit{EC-CRB}. The main purposes of this section are to show the power of erasure coding and introduce the notations.

%the erasure coding-based (EC-based) reliable broadcast that tolerates crash failures, namely .



\subsection{Erasure Coding-based Crash-tolerant RB}
%This works as long as $k \geq f$. 

We present our algorithms here. Source's logic is simple and its code is presented in Algorithm \ref{alg:EC-CRB-source}. To send a message $m$ in round with index $h$, it encodes the message $m$ and then disseminates to each peer. The message is a tuple that contains the tag $\msg$, the source identifier $s$, corresponding coded element, and round index $h$. 

To deal with asynchrony and failures, our algorithm is event-driven, similar to prior algorithms \cite{Bracha:1987:ABA:36888.36891,Raynal18}. 
The pseudo-code for peers and the source when receiving a message from the sender $j$ is presented in Algorithm \ref{alg:EC-CRB-peer}. 
First, upon receiving a coded element from the source, node $i$ forwards an $\echo$ message along with the coded element. Second, upon receiving an $\echo$ message, node $i$ decodes the message if it has received enough number of coded elements. 

The key design behind how crash-tolerant RB achieves the all-or-nothing property is that each peer needs to (pessimistically) help deliver the message to other peers. EC-CRB achieves this at Line \ref{line:crash-helper} in Algorithm \ref{alg:EC-CRB-peer}.
There are several designs that affect the complexity. %Please refer to Appendix \ref{XXX} for more discussion.

%\lewis{ Algorithm 4 is necessary to help other non-faulty peer receive the message, and  has several different ways of implementation. One other is to use request idea like the Byzantine version. Here I just choose the simplest one. The other version is waiting until $\ctr[] \geq k+f$ so that others are guaranteed to receive enough coded elements. There might be some interesting trade-off, e.g., resilience, number of rounds, message complexity.}





==> pre.tex <==
%\section{Preliminaries}

%\lewis{The text in this file should be merged with model section.}

%\paragraph{System}

\commentOut{++++++++++++++++
\section{Notations}
For each message $m$ that a correct server $j$ wants all correct servers to reliably accept, $m$ is associated with an index $h$, and thus $m$ can be uniquely indexed through a tuple $(j, h)$ in the system due to the message authentication assumption discussed above. 
In a synchronous system, $m$ is the message that $j$ sends at $h$-th reliable broadcast;
In the distributed data store context, $h$ could be the key of the message or a serial number associated with the message.

We use $\texttt{S}_i[j, h]$ to denote the set of messages that the server $i$ collects, in which are candidates that can be identified with $(j, h)$.
When the context is clear, we omit the subscript $i$. 

We use $\texttt{Counter}[*]$ to denote a local counter of messages that is initialized to 0.

We use $\mathbb{H}(*)$ to denote the cryptographic hash function. When we say a server sends a message to all servers, we assume it also sends to itself.
++++++++++}

